Spectral action and heat kernel trace for Ricci flat manifolds from stochastic flow over second quantized $L^2$-differential forms

A quantum stochastic differential equation (qsde) on Fock space over $L^2$ differential 1-forms is given from the small "time" flow of which the trace of the connection Laplacian heat kernel for the spinor endomorphism bundle can be computed over any compact Ricci-flat Riemannian manifold. The existence of the stochastic flow is established by adapting the construction from [14]. When the manifold supports a parallel spinor - Ricci-flatness is a required integrability condition for parallel spinors, the trace of Dirac Laplacian heat kernel of the spinor bundle can be recovered. For 4-manifolds, this corresponds to the spectral action, and realizes Einstein-Hilbert action as a stochastic flow.

==> lib/header_v1.tex <==
\usepackage{fancyhdr}
\pagestyle{fancy}
%\pagestyle{empty}
\renewcommand{\headrulewidth}{0pt} % get rid of line under header
\usepackage[bottom]{footmisc} % \usepackage[bottom,norule]{footmisc}
\fancyhf{}
\usepackage{lastpage}
\fancyfoot[R]{\small{\url{home}} \thepage/\pageref{LastPage}}
%\fancyfoot[R]{\small{\textsc{DocumentTitle}}}
%\fancyfoot[L]{\small{\url{127.0.0.1}}}
%\fancyhead[R]{\small{\textsc{DocumentTitle}}}
